Taming Consistency Distillation for Accelerated Human Image Animation

Recent advancements in human image animation have been propelled by video diffusion models, yet their reliance on numerous iterative denoising steps results in high inference costs and slow speeds. An intuitive solution involves adopting consistency models, which serve as an effective acceleration paradigm through consistency distillation. However, simply employing this strategy in human image animation often leads to quality decline, including visual blurring, motion degradation, and facial distortion, particularly in dynamic regions. In this paper, we propose the DanceLCM approach complemented by several enhancements to improve visual quality and motion continuity at low-step regime: (1) segmented consistency distillation with an auxiliary light-weight head to incorporate supervision from real video latents, mitigating cumulative errors resulting from single full-trajectory generation; (2) a motion-focused loss to centre on motion regions, and explicit injection of facial fidelity features to improve face authenticity. Extensive qualitative and quantitative experiments demonstrate that DanceLCM achieves results comparable to state-of-the-art video diffusion models with a mere 2-4 inference steps, significantly reducing the inference burden without compromising video quality. The code and models will be made publicly available.

==> sec/X_suppl_arxiv.tex <==
\clearpage



\twocolumn[
% \maketitlesupplementary
{
% \maketitle
% \twocolumn[
        \centering
        \Large
        \textbf{\thetitle}\\
        \vspace{0.3em}Supplementary Material \\
        \vspace{1.5em}
    \centering
    \vspace{5pt}
    % \includegraphics[width=0.99\textwidth]{Picture/first_figure_small.pdf}
    \includegraphics[width=1.00\textwidth]{Picture_supp/Compare_mv_small.pdf}
    \vspace{-28pt}
    \captionof{figure}{
        \textbf{Qualitative comparison on compositional motion-to-video synthesis}. The videos are generated by taking textual descriptions
and motion vectors as conditions. Compared to VideoComposer, TF-T2V produces more realistic and appealing results.
        %
        % Since only language-free videos are required, High-definition videos can be easily generated.
        % High-definition videos can be 
        %
    }
    \label{first_figure_supp}
    \vspace{18pt}
    }
    %
]

% \end{figure*}

% Due to page limitations, we move some parts
Due to the page limit of the main text, we add more details and experimental results in this appendix.
%
% In addition, 
Besides,
limitations and future work will also be discussed.
%


\begin{table}[t]
    % \vspace{-1.1em}
    \caption{
        {
        Ablation study on different training manners. 
        % 
    }}
     \label{tab:compare_with_train_manner}
     \vspace{-3mm}
    \tablestyle{4pt}{0.95}
    % \vspace{-5pt}
    \centering
    % \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{10pt}{
   % \begin{tabular}{@{}lc@{}}
   % \resizebox{\textwidth}{20mm}{
   % \scalebox{0.98}{
      \begin{tabular}{l|ccc}
    \shline
        Setting       &  FID ($\downarrow$) &   FVD  ($\downarrow$)  & CLIPSIM ($\uparrow$) \\
        \shline
      
        %
        Separately   &  9.22 & 503 & 0.2905 \\
        \rowcolor{Gray}
        Jointly  &   \textbf{8.19}  & \textbf{441}  & \textbf{0.2991}  \\
        % \shline
       \shline
 %      
%
    \end{tabular}
    }
    % \vspace{-10pt}
    \vspace{-3mm}
% \end{wraptable}
\end{table}

\section{More experimental details}

In \cref{first_figure_supp}, we show the comparison on compositional motion-to-video synthesis.
%
\method achieves more appealing results than the baseline VideoComposer.
%
Following prior works, 
%
we use an off-the-shelf pre-trained variational
autoencoder (VAE) model from Stable Diffusion 2.1 to encode the latent features.
The VAE encoder has a downsample factor of 8.
% The model structure of A is basically the same as that of B and C to facilitate fair comparison.
%
In the experiment,
the network structure of \method is basically consistent with the open source ModelScopeT2V and VideoComposer to facilitate fair comparison.
%
Note that \method is a plug-and-play framework that can also be applied to other text-to-video generation and controllable video synthesis methods.
%
% To verify the high-definition generation capability of \method, we train 
% To verify that \method can be extended to high-definition video generation, we also use text-free videos to train a high-resolution text-to-video model, such as $896\times512$. For high-definition compositional video synthesis, we synthesize $1280\times640$ and $1280\times768$ videos to demonstrate the excellent application potential of our method.
%
% \method support different resolutions as input
% As for human evaluation, we randomly generated 100 videos and asked users to 
% [Details about user study]
For human evaluation, we randomly generate 100 videos and ask users to rate and evaluate them. The highest score for each evaluation content is 100\%, the lowest score is 0\%, and the final statistical average is reported.




\section{Additional ablation study}

